A Proof of Correctness for the Tardis Cache Coherence Protocol

We prove the correctness of a recently-proposed cache coherence protocol, Tardis, which is simple, yet scalable to high processor counts, because it only requires O(logN) storage per cacheline for an N-processor system. We prove that Tardis follows the sequential consistency model and is both deadlock- and livelock-free. Our proof is based on simple and intuitive invariants of the system and thus applies to any system scale and many variants of Tardis.

==> tso.tex <==
\subsection{Other Consistency Models}

In \cref{sec:proof}, we proved that the Tardis protocol follows 
sequential consistency. In this section, we show that Tardis also 
supports relaxed consistency models. We use TSO as an example, which 
is defined in Definition~\ref{def:tso} (\cite{sorin2011}).

\begin{definition}[TSO] \label{def:tso} An execution of a program 
follows TSO iff

	{\bf Rule 1:} $\forall$ address a, b from the same processor, 
	$L(a) <_p L(b) \Rightarrow L(a) <_m L(b)$,
	$L(a) <_p S(b) \Rightarrow L(a) <_m S(b)$,
	$S(a) <_p S(b) \Rightarrow S(a) <_m S(b)$.

	{\bf Rule 2:} {\it Value of} $L$($a$) = {\it Value of 
Max}$_{<m}\{S(a) | S(a) <_m L(a) \vee S(a) <_p L(a)\}$
\end{definition}

We define the following processor model for TSO consistency model. 

\begin{definition}[TSO Processor] \label{def:tso-proc}
$\forall$ address a, b, $L(a) <_p L(b) \Rightarrow L(a) \leq_{ts} L(b) 
\wedge L(a) <_p S(b) \Rightarrow L(a) \leq_{ts} S(b) \wedge S(a) <_p 
S(b) \Rightarrow S(a) \leq_{ts} S(b)$.
$\forall X, Y \in \{Ld, St\}$, $X <_p Y \Rightarrow X <_{pt} Y$
\end{definition}

Using similar proof techniques for sequential consistency, we can 
prove that the Rule 1 in Definition~\cref{def:tso} is obeyed. However, 
for Rule 2, we can only prove that $\{S(a) | S(a) <_{ts} L(a)\} =
\{ S(a) | S(a) <_m L(a)\}$ which means Tardis only expresses a subset 
of the TSO model. In order to express the whole TSO model, we need to 
change the {\it LoadHit} and {\it L1Miss} rules in 
\cref{tab:l1-rules}. Specifically, if the cacheline is in \M state in 
L1, a load request is always considered a hit regardless of the 
timestamps. The timestamp of the load is then the \pts in the request.  
With this modification, we can prove the following invariant which can 
then be proven to be equivalent to Rule 2 in Definition~\ref{def:tso}. 

\[ {\it Value\;of}\;L(a) = \textit{Value\;of\; Max}_{<ts} \{ S(a) | 
S(a) \leq_{ts} L(a) \vee S(a) <_p L(a) \}\] 


